On discretely structured growth models and their moments

The logistic equation is ubiquitous in applied mathematics as a minimal model of saturating growth. Here, we examine a broad generalisation of the logistic growth model to discretely structured populations, motivated by examples that range from the ageing of individuals in a species to immune cell exhaustion by cancerous tissue. Through exploration of a range of concrete examples and a general analysis of polynomial kinetics, we derive necessary and sufficient conditions for the dependence of the kinetics on structure to result in closed, low-dimensional moment equations that are exact. Further, we showcase how coarse-grained moment information can be used to elucidate the details of structured dynamics, with immediate potential for model selection and hypothesis testing. This paper belongs to the special collection: Problems, Progress and Perspectives in Mathematical and Computational Biology.

==> preamble.tex <==
\newcommand{\note}[1]{{\color{red}#1}}
\newcommand{\diff}[2]{\frac{\mathrm{d}#1}{\mathrm{d}#2}}
\let\olddeg\deg
\renewcommand{\deg}[1]{\olddeg{(#1)}}
\newcommand{\constant}{\text{const.}}
\renewcommand{\vec}[1]{\bm{#1}}
\newcommand{\bjw}[1]{{\color{blue}{BJW: #1}}}
\newcommand{\changed}[1]{{\color{blue}#1}}
% \newcommand{\changed}[1]{{#1}}
